Covariant Compositional Networks For Learning Graphs

Most existing neural networks for learning graphs address permutation invariance by conceiving of the network as a message passing scheme, where each node sums the feature vectors coming from its neighbors. We argue that this imposes a limitation on their representation power, and instead propose a new general architecture for representing objects consisting of a hierarchy of parts, which we call Covariant Compositional Networks (CCNs). Here, covariance means that the activation of each neuron must transform in a specific way under permutations, similarly to steerability in CNNs. We achieve covariance by making each activation transform according to a tensor representation of the permutation group, and derive the corresponding tensor aggregation rules that each neuron must implement. Experiments show that CCNs can outperform competing methods on standard graph learning benchmarks.

==> tbl-HCEP.tex <==
\begin{table}[]
\centering
\caption{\label{tbl: HCEP}HCEP Results }
\begin{tabular}{||c | c | c | c | c | c | c | c ||}
	\hline
	Method & Train MAE & Train RMSE & Test MAE & Test RMSE \\
	\hline\hline
	Lasso & 0.863 & 1.190 & 0.867 & 1.437 \\
	\hline
	Ridge Regression & 0.849 & 1.164 & 0.854 & 1.376 \\
	\hline
	Random Forest & 0.999 & 1.331 & 1.004 & 1.799 \\
	\hline
	Gradient Boosted Tree & 0.676 & 0.939 & 0.704 & 1.005 \\
	\hline
	Weisfeiler-Lehman Graph Kernel & 1.206 & 1.587 & 1.201 & 1.568 \\
	\hline
	Molecular Graph Fingerprint & 0.848 & 1.187 & 0.851 & 1.177 \\
	\hline
	First order steerable message passing & \textbf{0.506} & \textbf{0.762} & \textbf{0.516} & \textbf{0.771} \\
	\hline
	 Second order steerable message passing& 0.548 & 0.819 & 0.556 & 0.821 \\
	\hline
\end{tabular}
\end{table}


